Dataset-On-Demand: Automatic View Search and Presentation for Data Discovery

Many data problems are solved when the right view of a combination of datasets is identified. Finding such a view is challenging because of the many tables spread across many databases, data lakes, and cloud storage in modern organizations. Finding relevant tables, and identifying how to combine them is a difficult and time-consuming process that hampers users' productivity. In this paper, we describe Dataset-On-Demand (DoD), a system that lets users specify the schema of the view they want, and have the system find views for them. With many underlying data sources, the number of resulting views for any given query is high, and the burden of choosing the right one is onerous to users. DoD uses a new method, 4C, to reduce the size of the view choice space for users. 4C classifies views into 4 classes: compatible views are exactly the same, contained views present a subsumption relationship, complementary views are unionable, and contradictory views have incompatible values that indicate fundamental differences between views. These 4 classes permit different presentation strategies to reduce the total number of views a user must consider. We evaluate DoD on two key metrics of interest: its ability to reduce the size of the choice space, and the end to end performance. DoD finds all views within minutes, and reduces the number of views presented to users by 2-10x.

==> sections/discussion.tex <==
\section{Discussion}

\notera{shorten}

One fundamental difference of Aurum-DoD with respect to previous efforts to
assemble views for users, is that it merges the mapping and view selection
problem together. Instead of relying on users to create mappings manually, or
select automatically suggested mappings, Aurum-DoD instead assembles all
possible mappings. This is a good idea because although sometimes mappings
will be wrong due to data quality issues or due to an incorrect inclusion
dependency, multiple mappings may also exist with different semantics. In both
cases, humans are better tailored to choose the view that satisfies their needs. 

We have identified a number of additional consequences of Aurum-DoD's design
which we have not exploited in this paper but are worth mentioning here as
avenues of future work:

\begin{myitemize}
\item\textbf{Focus on high-value tables} As the amount of tables that companies
accumulate grows, their governance (documentation, quality control, etc.)
becomes harder and harder. A history of query views submitted from users to
Aurum-DoD produces a rich log of tables that were involved in the assembling of
views. Because the views were requested by actual users, the collection of
tables indicates highly-valuable tables. This can be used to prioritize where to
dedicate preparation/governance effort.
\item\textbf{Beam data preparation} Similar to how we know what tables appear
more often in the assembly of views, we know what tables DoD tries to join
unsuccessfully. These cases provide an input for transformation algorithms,
which can be used to identify transformations to the tables so they join with
each other. The advantage of DoD in this case is on highlighting what tables are
worth joining, as trying to learn transformations across \emph{all} tables is
not possible.
\item\textbf{Find PKFK} Aurum-DoD relies on Aurum's ability to identify
inclusion dependencies automatically across many data sources. No information
from users is necessary, however, some of the inclusion dependencies won't be
real PKFKs. The 4C algorithm means that those wrong views will be ultimately
detected by users. However, it also demands more compute cycles that are not
dedicated to useful work. Therefore, although Aurum-DoD presents a practical way
of dealing with approximate PKFKs, in an automatic way, more research to
identify better quality PKFK will be welcome.
\item\textbf{Trustworthiness, cleanliness} People's relationship with data is
many times subjective: a user may trust more a view because it recognizes some
of its data, a view that is dirty to some user is clean to another. Aurum-DoD
does not make any decision on either the trustworthiness or cleanliness of views
and instead offers an efficient way of navigating them. However, it is
possible to include more metadata while the views are being assembled to help
users make their subjective calls.
\end{myitemize}

All in all, we think Aurum-DoD, as a system, provides an alternative way of
performing end to end data preparation. In this paper, we present a first step
in the automatic assembly of SPJ queries from an input query view definition,
and the organization of the output results for easy human and machine
consumption.

